Unified-IO 2: Scaling Autoregressive Multimodal Models with Vision, Language, Audio, and Action

We present Unified-IO 2, the first autoregressive multimodal model that is capable of understanding and generating image, text, audio, and action. To unify different modalities, we tokenize inputs and outputs -- images, text, audio, action, bounding boxes, etc., into a shared semantic space and then process them with a single encoder-decoder transformer model. Since training with such diverse modalities is challenging, we propose various architectural improvements to stabilize model training. We train our model from scratch on a large multimodal pre-training corpus from diverse sources with a multimodal mixture of denoisers objective. To learn an expansive set of skills, such as following multimodal instructions, we construct and finetune on an ensemble of 120 datasets with prompts and augmentations. With a single unified model, Unified-IO 2 achieves state-of-the-art performance on the GRIT benchmark and strong results in more than 35 benchmarks, including image generation and understanding, natural language understanding, video and audio understanding, and robotic manipulation. We release all our models to the research community.

==> table/grit_vqa.tex <==
\begin{table}
    \small
    \centering
    
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{l|ccccc}
        \toprule
          & all & sameSrc & newSrc & undist. & dist. \\ 
         \midrule
         \uiot{} &  71.5 & \textbf{84.4} & 58.5 & \textbf{87.2} & 78.2 \\
         \uio{} & \textbf{74.5} & 81.7 & \textbf{67.24} & 85.4 & \textbf{79.0} \\
         GPV 2 & 63.2 & 73.8 & 52.7 & 75.2 & 65.3 \\
        \bottomrule
    \end{tabular}}
    \caption{Scores on different subset of the GRIT VQA test corpus, include the same-source and new-source set and the distorted and un-distorted sets.}
    \label{tab:grit_vqa}    
\end{table}


==> table/multi_task_1.tex <==
\begin{table*}[tb]
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.25}
\center
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l c  c c c c c  c c  c c c c}
\toprule


\midrule
 & \rotatebox{90}{\raisebox{0.5pt}{HellaSwag}}
 & \rotatebox{90}{\raisebox{0.5pt}{ImageNet}} 
 & \rotatebox{90}{\raisebox{0.5pt}{TIFA}} 
 & \rotatebox{90}{\raisebox{0.5pt}{MagicBrush}} 
 & \rotatebox{90}{\raisebox{0.5pt}{UCF101}} 
 & \rotatebox{90}{\raisebox{0.5pt}{SEED-Bench}} 
 & \rotatebox{90}{\raisebox{0.5pt}{VGG-Sound}} 
 & \rotatebox{90}{\raisebox{0.5pt}{AudioCaps}} 
 & \rotatebox{90}{\raisebox{0.5pt}{COCO}} 
 & \rotatebox{90}{\raisebox{0.5pt}{NYUv2}} 
 & \rotatebox{90}{\raisebox{0.5pt}{Objectron}} 
 & \rotatebox{90}{\raisebox{0.5pt}{VIMA-Bench}}

%  & \rotatebox{90}{\raisebox{0.5pt} -}
%  & \rotatebox{90}{\raisebox{0.5pt} -} 
%  & \rotatebox{90}{\raisebox{0.5pt} -} 
 \\

 \midrule
 Split & test & val & test & single-turn test & test & test & test & test & val & val & test & test\\
 Metric & Acc.$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & CLIP-I$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & FAD$\downarrow$ & mAP$\uparrow$ & RMSE$\downarrow$ & AP$_{\text{3D}}$$\uparrow$ & Succ.$\uparrow$ \\
 \midrule 
 Unified SOTA & - & - & - & - & - & - & - & - & - & - & - & - \\
   & - & - & - & - & - & - & - & - & - & - & - & - \\
 \midrule
UIO-2 1B & - & - & - & - & - & - & - & - & - & - & - & -\\
UIO-2 3B & - & - & - & - & - & - & - & - & - & - & - & -\\
UIO-2 7B & - & - & - & - & - & - & - & - & - & - & - & -\\
 \midrule
 Single or fine- & - & - & - & - & - & - & - & - & - & - & - & - \\
 tuned SOTA  &- & - & - & - & - & - & - & - & - & - & - & - \\

\bottomrule
\end{tabular}
}
\caption{\small{Comparison with SOTA methods on 12 benchmarks. \uiot{} achieves competitive performance against specialized and benchmark fine-tuned state-of-the-art models on a broad range of tasks: NLU (HellaSwag~\cite{zellers2019hellaswag}), image classification (ImageNet~\cite{deng2009imagenet}), text-to-image generation (TIFA~\cite{hu2023tifa}), image editing (MagicBrush~\cite{zhang2023magicbrush}), video classification (UCF101~\cite{soomro2012ucf101}), vision and language (SEED-Bench~\cite{li2023seed}), audio classification (VGG-Sound~\cite{chen2020vggsound}), text-to-audio generation (AudioCaps~\cite{audiocaps}), object detection (COCO~\cite{coco}), object segmentation (NYUv2~\cite{nyu_depth}), 3d object detection (Objectron~\cite{ahmadyan2021objectron}), and robot manipulation (VIMA-Bench~\cite{jiang2023vima}). Acc.: top-1 accuracy, CLIP-I: CLIP~\cite{radford2021learning} cosine similarity between the generated image and ground-truth, FAD: Fr\'echet Audio Distance~\cite{Kilgour2019Fr}, Succ.: success rate.
}}
\label{tab:multi_task_1}

\end{table*}

==> table/multi_task_2.tex <==
\begin{table}[htbp!]
\small
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{l | l | l | c c c | c}
\toprule
Input & Output & Data & 1B & 3B & 7B  & SOTA \\ \hline

text & \multirow{2}{*}{image} & TIFA$\uparrow$~\cite{hu2023tifa}  & 74.2 & 79.2 & 80.6 & 82.0~\cite{SD15} \\
\cline{1-1}
\cline{3-7}

i+t & & MagicBrush$\uparrow$~\cite{zhang2023magicbrush} & 0.290 & 0.295 & 0.297 & 0.278~\cite{zhang2023magicbrush} \\

\hline

text & audio & AudioCaps$\downarrow$~\cite{audiocaps} & 3.02 & 2.79 & 2.87 & \\

\hline

action & action & VIMA-Bench$\uparrow$~\cite{jiang2023vima} & 48.4 & 54.6 & 56.4 & \\

\hline

image & sparse & NYUv2$\downarrow$~\cite{nyu_depth} & & & & \\

\hline

\multirow{3}{*}{i+t} & \multirow{3}{*}{dense} & RefCOCO$\uparrow$~\cite{referitgame} & & & 90.0 & 87.5~\cite{you2023ferret}  \\
 & & RefCOCO+$\uparrow$~\cite{referitgame} & & & 81.8 & 80.8~\cite{you2023ferret} \\
 & & RefCOCOg$\uparrow$~\cite{mao2016generation} & & & 85.7 & 83.93~\cite{you2023ferret} \\

\hline

\multirow{6}{*}{text} & \multirow{27}{*}{text} & HellaSwag$\uparrow$~\cite{zellers2019hellaswag} & 38.9 & 49.5 & 53.3 & \\
 & & MMLU$\uparrow$~\cite{hendrycks2021measuring} & 27.9 & 29.5 & 30.1 & \\
 & & ArcEasy$\uparrow$~\cite{clark2018think} & 41.6 & 49.2 & 53.5 & \\
 & & ArcChallenge$\uparrow$~\cite{clark2018think} & 26.5 & 29.4 & 34.0 & \\
 & & BoolQ$\uparrow$~\cite{clark2019boolq} & 66.7 & 73.7 & 77.0 & \\
 & & Big-bench$\uparrow$~\cite{srivastava2023beyond} & 32.3 & 34.4 & 35.8 & \\

\cline{1-1}
\cline{3-7}

\multirow{2}{*}{image} & & ImageNet$\uparrow$~\cite{deng2009imagenet} & 73.7 & 76.9 & 78.7 & \\
      &      & COCO Captions$\uparrow$~\cite{chen2015microsoft} & & 128.7 & & \\

\cline{1-1}
\cline{3-7}

\multirow{8}{*}{i+t} & & VQAv2$\uparrow$~\cite{balanced_vqa_v2} &  & 77.2 & 78.9 & 78.5~\cite{llava15} \\
    &      & VizWizVQA$\uparrow$~\cite{gurari2018vizwiz} & & 55.4 & & \\
    &      & OK-VQAv2$\uparrow$~\cite{reichman2023outside} & 42.2 & 47.0 & 50.2 & \\
    &      & TallyQA$\uparrow$~\cite{acharya2019tallyqa} & 69.1 & 72.2 & 74.4 & \\
    &      & GQA$\uparrow$~\cite{hudson2019gqa} & & 65.0 & & \\
    &      & TextVQA$\uparrow$~\cite{singh2019towards} & & 40.1 & & \\
    &      & ScienceQA$\uparrow$~\cite{lu2022learn} & & 88.6 & 88.9 & \\
    &      & SEED-S$\uparrow$~\cite{li2023seed} & 55.1 & 63.8 & 65.5 & 58.2~\cite{bai2023qwen} \\

\cline{1-1}
\cline{3-7}

\multirow{7}{*}{video} & & UCF101$\uparrow$~\cite{soomro2012ucf101} & 82.0 & 86.5 & 89.5 & \\
      &      & VATEXCaption$\uparrow$~\cite{wang2019vatex} & 39.0 & 42.7 & 45.4 & \\
      &      & MSR-VTT$\uparrow$~\cite{xu2016msr} & 45.1 & 49.1 & 49.0 & \\
      &      & MSRVTT-QA$\uparrow$~\cite{xu2017video} & 41.5 & 40.6 & 42.0 & \\
      &      & MSVD-QA$\uparrow$~\cite{xu2017video} & 50.5 & 50.9 & 52.6 & \\
      &      & STAR$\uparrow$~\cite{wu2021star} & 52.4 & 52.7 & 53.0 & \\
      &      & SEED-T$\uparrow$~\cite{li2023seed} & 34 & 44.2 & 46 & 39.8~\cite{ye2023mplug_owl2}  \\
      &      & SEED-All$\uparrow$~\cite{li2023seed} & 49.6 & 58.7 & 60.4 & 58.6~\cite{llava15}  \\

\cline{1-1}
\cline{3-7}

\multirow{3}{*}{audio} &  & VGG-Sound$\uparrow$~\cite{chen2020vggsound} & 36.6 & 43.1 & 46.7 & \\
      &  & AudioCaps$\uparrow$~\cite{audiocaps} & & & & \\
      &  & Clotho$\uparrow$~\cite{drossos2020clotho} & 22.9 & 25.0 & 27.8 & \\

\cline{1-1}
\cline{3-7}

a+v & & Kinetics-Sounds$\uparrow$~\cite{arandjelovic2017look} & 86.6 & 88.0 & 89.3 \\

\bottomrule


\end{tabular}}
\caption{Comparison with SOTA methods.}
\label{tab:multi_task_2}
\end{table}

%(Acc.$\uparrow$)
%(CLIP-T$\uparrow$)

==> table/multi_task_new.tex <==
\begin{table*}[tb]
\tablefont
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.25}
\center
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l c  c c c c c  c c  c c c c}
\toprule


\midrule
 & \rotatebox{90}{\raisebox{0.5pt}{HellaSwag}}
 & \rotatebox{90}{\raisebox{0.5pt}{ImageNet}} 
 & \rotatebox{90}{\raisebox{0.5pt}{TIFA}} 
 & \rotatebox{90}{\raisebox{0.5pt}{MagicBrush}} 
 & \rotatebox{90}{\raisebox{0.5pt}{UCF101}} 
 & \rotatebox{90}{\raisebox{0.5pt}{SEED-Bench}} 
 & \rotatebox{90}{\raisebox{0.5pt}{VGG-Sound}} 
 & \rotatebox{90}{\raisebox{0.5pt}{AudioCaps}} 
 & \rotatebox{90}{\raisebox{0.5pt}{COCO}} 
 & \rotatebox{90}{\raisebox{0.5pt}{NYUv2}} 
 & \rotatebox{90}{\raisebox{0.5pt}{Objectron}} 
 & \rotatebox{90}{\raisebox{0.5pt}{VIMA-Bench}}

%  & \rotatebox{90}{\raisebox{0.5pt} -}
%  & \rotatebox{90}{\raisebox{0.5pt} -} 
%  & \rotatebox{90}{\raisebox{0.5pt} -} 
 \\

 \midrule
 Split & test & val & test & single-turn test & test & test & test & test & val & val & test & test\\
 Metric & Acc.$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & CLIP-I$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & Acc.$\uparrow$ & FAD$\downarrow$ & mAP$\uparrow$ & RMSE$\downarrow$ & AP$_{\text{3D}}$$\uparrow$ & Succ.$\uparrow$ \\
 \midrule 
 Unified SOTA & - & - & - & - & - & - & - & - & - & - & - & - \\
   & - & - & - & - & - & - & - & - & - & - & - & - \\
 \midrule
UIO-2 1B & - & - & - & - & - & - & - & - & - & - & - & -\\
UIO-2 3B & - & - & - & - & - & - & - & - & - & - & - & -\\
UIO-2 7B & - & - & - & - & - & - & - & - & - & - & - & -\\
 \midrule
 Single or fine- & - & - & - & - & - & - & - & - & - & - & - & - \\
 tuned SOTA  &- & - & - & - & - & - & - & - & - & - & - & - \\

\bottomrule
\end{tabular}
}
\caption{}
\label{tab:multi_task_1}

\end{table*}

==> table/pretrain_qualitive.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]
\tablefont
\footnotesize
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.15}
\center
\resizebox{\textwidth}{!}{
\begin{tabular}{p{6cm} @{\hspace{0.1cm}} p{3cm} @{\hspace{0.1cm}} C{3cm}}
\toprule
Model Inputs & & Model Response \\
\midrule
 A video of a \textit{man} (\textit{woman}) saying \uiot~is a model that works with vision, language, audio, and action.  &  &  \href{https://ai2-prior-uio.s3.us-west-2.amazonaws.com/public/samples/tts_output_1.wav}{\faVolumeUp} (\href{https://ai2-prior-uio.s3.us-west-2.amazonaws.com/public/samples/tts_output_1.wav}{\faVolumeUp}) \\
A video of a man playing guitar. & \parbox[c]{1em}{\includegraphics[width=0.7in]{figure/piano.pdf}}  & \href{https://ai2-prior-uio.s3.us-west-2.amazonaws.com/public/samples/tts_output_1.wav}{\faVolumeUp} \\
\midrule

\bottomrule
\end{tabular}}
\caption{}
\label{tab:pretrain-qualitive}
\end{table*}



==> table/task.tex <==
% What method should we list in table 1?

% LLM based model 

\begin{table*}[t]
\label{tasks}
\renewcommand{\dashlinedash}{2pt}
\renewcommand{\dashlinegap}{2pt}
\newcommand{\checkcol}{p1.5cm}
\newcolumntype{M}{>{\centering\arraybackslash}p{1.0 cm}}
\renewcommand{\indent}{\hspace{0.2cm}}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.25}
\center
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l M M M M M M M M M : M M M M M M }
  \toprule
  & \multirow{2}{1.3cm}{Train from Scratch} & \multirow{2}{1.3cm}{Instr. Fine-tuned} & \multicolumn{7}{c}{Input Modalities} & \multicolumn{6}{c}{Output Modalities} \\ 
    \cmidrule(r){4-10}
    \cmidrule(r){11-16}
  & & & Text & Image & Audio & Video & \textit{Action} & \textit{Sparse} & \multicolumn{1}{c}{\textit{Dense}} & Text & Image & Audio & \textit{Action} & \textit{Sparse} & \multicolumn{1}{c}{\textit{Dense}} \\
  \midrule
Flamingo \cite{Alayrac2022FlamingoAV}  & - & \checkmark &  \checkmark 
 & \checkmark & - & \checkmark & - & - & - & \checkmark & - & - & - & - & - \\
\band LLAVA-1.5 \cite{llava15} & - & \checkmark & \checkmark & \checkmark & - & - & - & - & - & \checkmark & - & - & - & \checkmark & - \\
RT-2 \cite{brohan2023rt} \\

ImageBind LLM \cite{han2023imagebind} & \checkmark & - & \checkmark & \checkmark & \checkmark & \checkmark & - & - & \checkmark & \checkmark & - & - & - & - & - \\
\midrule
CoDi \cite{tang2023codi} & - & - & \checkmark & \checkmark & \checkmark &  \checkmark & - & - & - & \checkmark & \checkmark & \checkmark & - & - & - \\
\midrule
OFA \cite{wang2022OFA} & - & \checkmark & \checkmark & \checkmark & - & - & - & \checkmark & - & \checkmark & \checkmark & - & - & \checkmark & - \\ 
C3MLion \cite{} & \checkmark & \checkmark & \checkmark & - & - & - & \checkmark & - & \checkmark & - & - & - & \checkmark & - \\ 
Kosmos-2 & \checkmark & \checkmark & \checkmark & - & - & - & \checkmark & - & \checkmark & - & - & - & \checkmark & - \\
Unified-IO  & \checkmark & \checkmark & - & - & - & - & \checkmark & \checkmark & \checkmark & \checkmark & - & - & - & - \\
\band Unified-IO-2  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

 \bottomrule
\end{tabular}}

\caption{\small{List of the models with their supported input and output modalities. Unified-IO-2 is the first Unified model that support those output modalities without Task specific decoder.}}
\vspace{-0.15in}
\label{tab:tasks}
\end{table*}


==> table/tifa.tex <==
\begin{table*}[htbp!]
% \footnotesize
\small
\centering
\begin{tabular}{c c c c c | c c c | c c c | c c c}
\toprule
Type        & \multicolumn{4}{c}{Specialist} & \multicolumn{3}{c}{Generalist} & \multicolumn{3}{c}{\uiot{} Pretrain} & \multicolumn{3}{c}{\uiot{} FT} \\
\midrule
Model       & SD-1.1 &  minDALL-E & SD-1.5 & SD-2.1 & CoDi & OFA-L & Emu & 1B & 3B & 7B & 1B & 3B & 7B \\

Score       & 75.7                        & 79.4       & 78.4                   & 82.0                     & 71.6 & 69.50                & 65.5 & 70.2 & 77.2 & 78.7 & 74.3 & 80.0 & 81.3 \\
\bottomrule
\end{tabular}
\caption{TIFA TODO cite}
\label{tab:tifa}
\end{table*}

